Software Model Checking via Large-Block Encoding

The construction and analysis of an abstract reachability tree (ART) are the basis for a successful method for software verification. The ART represents unwindings of the control-flow graph of the program. Traditionally, a transition of the ART represents a single block of the program, and therefore, we call this approach single-block encoding (SBE). SBE may result in a huge number of program paths to be explored, which constitutes a fundamental source of inefficiency. We propose a generalization of the approach, in which transitions of the ART represent larger portions of the program; we call this approach large-block encoding (LBE). LBE may reduce the number of paths to be explored up to exponentially. Within this framework, we also investigate symbolic representations: for representing abstract states, in addition to conjunctions as used in SBE, we investigate the use of arbitrary Boolean formulas; for computing abstract-successor states, in addition to Cartesian predicate abstraction as used in SBE, we investigate the use of Boolean predicate abstraction. The new encoding leverages the efficiency of state-of-the-art SMT solvers, which can symbolically compute abstract large-block successors. Our experiments on benchmark C programs show that the large-block encoding outperforms the single-block encoding.

==> Makefile <==
# Makefile for papers
LATEX = pdflatex

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
all:
	@echo $(LATEX) main.tex </dev/null
	@if $(LATEX) main.tex </dev/null; then \
		true; \
	else \
		stat=$$?; touch main.dvi; exit $$stat; \
	fi 
	#bibtex main
	@echo $(LATEX) main.tex </dev/null
	@while grep "Rerun to get cross" main.log; do \
		echo $(LATEX) main.tex </dev/null; \
		if $(LATEX) main.tex </dev/null; then \
			true; \
		else \
			stat=$$?; touch main.dvi; exit $$stat; \
		fi; \
	done
	@if grep "miktex" main.log ; then \
		cygstart main.pdf; \
	fi

clean:
	rm -f main.aux main.log main.out main.ps main.pdf main.dvi main.blg *.bak *.auto


==> proof_efficiency.tex <==
\begin{proof}

Let $G_{\mathsf{loop}}$ be the set of loopback edges for $A$,
as computed by a standard DFS visit \cite{clr}. 
Let $L'$ be a reverse topological order of the vertices of the DAG $(L, G\setminus G_{\mathsf{loop}})$.
The algorithm can be described by the following pseudo-code:
%
\begin{small}
\begin{algorithmic}[1]
  \newcommand{\IN}{\textbf{in}\xspace}
  \newcommand{\NOT}{\textbf{not}\xspace}
  \newcommand{\FALSE}{\textbf{false}\xspace}
  \newcommand{\TRUE}{\textbf{true}\xspace}
  \newcommand{\SET}[2]{\STATE #1 := #2}
  \newcommand{\EACH}{\textbf{each}\xspace}
  \renewcommand{\algorithmiccomment}[1]{\emph{/* #1 */}}  
  \STATE apply Rule 0
  \FOR{\EACH $l$ \IN $L'$}
     \SET{done}{\FALSE}
     \WHILE{\NOT done}
        \IF{exists $\{(l, \op_1, l_1), (l_1, \op_2, l_2) \ldots (l_1, \op_n, l_n) \} \subseteq G$ for which Rule 1 is applicable}
           \STATE remove $l_1$ from $L$\\
           \STATE replace $\{(l, \op_1, l_1), (l_1, \op_2, l_2) \ldots (l_1, \op_n, l_n) \}$ with \\$\{(l, \op_1 \sequence \op_2, l_2) \ldots (l, \op_1 \sequence \op_n, l_n)\}$ in $G$ \\
           \COMMENT{apply Rule 1}
        \ELSIF{exists $\{(l, \op_1, l_1), (l, \op_2, l_1)\} \subseteq G$ for which Rule 2 is applicable}
           \STATE replace $\{(l, \op_1, l_1), (l, \op_2, l_1)\}$ with $\{(l, \op_1 \parallel \op_2, l_1)\}$ in $G$ \\
           \COMMENT{apply Rule 2}
        \ELSE
           \SET{done}{\TRUE}
        \ENDIF
     \ENDWHILE
  \ENDFOR        
\end{algorithmic}
\end{small}

We can prove that the resulting CFA~$A'$ is a summarization of $A$ 
(that is, that the algorithm performs all the possible Rule applications)
as follows.

\smallskip \noindent
Let $C\defas (V, E)$ be a CFA, $C' \defas (V', E')$ be its summarization, and 
$\{(V_i, E_i)\}_{i=0..n}$ be the sequence of CFAs obtained 
after the application of $i$ Rules, 
where $(V_0, E_0) \equiv (V, E)$ and $(V_n, E_n) \equiv (V', E')$.
We say that the $i+1$-th Rule application depends on the $i$-th one
if and only if the Rule applied at the $i+1$-th step 
was not applicable in any of the CFAs $(V_0, E_0) \ldots (V_{i-1}, E_{i-1})$.
In this case, we say that the Rule applied at step $i+1$ \emph{was triggered} 
by the Rule applied at step $i$.

We observe that there are only two cases in which 
the application of a Rule can trigger other Rule applications. In particular:
\begin{enumerate}
\item Rule 1 can trigger Rule 2 in this case:\\[1ex]
  \raisebox{1cm}{$a)$}\hspace{2em} 
  \scalebox{0.3}{\inputfig{rule1_triggers_rule2}}
\item Rule 2 can trigger Rule 1 in this case:\\[1ex]
  \raisebox{1.5cm}{$b)$}\hspace{2em} 
  \scalebox{0.3}{\inputfig{rule2_triggers_rule1_a}} 
\end{enumerate}

In cases $a)$ and $b)$, the new Rule applications will be discovered 
and performed in the \textbf{while} loop of the above algorithm,
when processing $l_1$.

In case $c)$, after Rule 2 is applied to 
$\{(l_2, \op_2, l_3), (l_2, \op_3, l_3)\}$,
Rule 1 becomes applicable to
$\{(l_1, \op_1, l_2), (l_2, \op_2 \parallel \op_3, l_3), \ldots\}$.
Since the applicability condition of Rule 1 ensures 
that $(l_1, \op_1, l_2)$ is not a loopback edge, 
$l_1$ follows $l_2$ in the reverse topological order $L'$ 
(generated from $(L, G\setminus G_{\mathsf{loop}})$).
Therefore, Rule 1 will be applied 
in the \textbf{while} loop of the above algorithm
when processing $l_1$.

\medskip \noindent
We show that the time complexity is in $O(|L|+|G|)$ as follows.

Since each Rule application removes one edge from $G$, 
there can be at most $|G|$ Rule applications overall, 
therefore the body of the inner \textbf{while} loop is executed at most $|G|$ times.
Each operation in the \textbf{while} body can be executed in constant time, 
\footnote{This is true under the assumption
that there is a constant upper bound on the number of outgoing edges for each node.
Such assumption is valid for CFAs built from standard sequential programs, 
since each node has at most two outgoing edges, 
corresponding to the two branches of an if-then-else 
(\texttt{switch} statements are converted upfront into nested \texttt{if}s).}
given a suitable representation for $L$ and $G$.
The body of the \textbf{for} loop is executed $|L|$ times. 
Finally, the construction of $G_{\mathsf{loop}}$ 
and the reverse topological order $L'$ 
can be done in $O(|L|+|G|)$ time \cite{clr}.
Therefore, the whole algorithm can be executed in $O(|L|+|G|)$ time.
\qed
\end{proof}

